Deep Active Learning for Named Entity Recognition

Deep learning has yielded state-of-the-art performance on many natural language processing tasks including named entity recognition (NER). However, this typically requires large amounts of labeled data. In this work, we demonstrate that the amount of labeled training data can be drastically reduced when deep learning is combined with active learning. While active learning is sample-efficient, it can be computationally expensive since it requires iterative retraining. To speed this up, we introduce a lightweight architecture for NER, viz., the CNN-CNN-LSTM model consisting of convolutional character and word encoders and a long short term memory (LSTM) tag decoder. The model achieves nearly state-of-the-art performance on standard datasets for the task while being computationally much more efficient than best performing models. We carry out incremental active learning, during the training process, and are able to nearly match state-of-the-art performance with just 25\% of the original training data.

==> exps/exp-1.tex <==
\begin{figure*}[h]
  \centering
  \begin{subfigure}[t]{0.4\textwidth}
     \centering
%      \includegraphics[width=\linewidth]{active-eng-v2.pdf}
{\small
\begin{tikzpicture}[scale=1]
	\begin{axis}[mark repeat=4, 
    legend pos=south east,
    legend style={nodes={scale=0.5, transform shape}},
        width=1.2\textwidth,
        height=0.9\textwidth,
		xlabel={Percent of words annotated},
		ylabel={Test F1 score}, xmin=-5, xmax=85]
	\addplot coordinates {(2.838235,74.130000) (4.676471,78.670000) (6.514706,81.320000) (8.352941,82.000000) (10.191176,83.170000) (12.029412,83.570000) (13.867647,84.220000) (15.705882,84.250000) (17.544118,84.990000) (19.382353,85.210000) (21.220588,85.590000) (23.058824,85.900000) (24.897059,86.130000) (26.735294,86.130000) (28.573529,86.130000) (30.411765,86.130000) (32.250000,86.130000) (34.088235,86.140000) (35.926471,86.140000) (37.764706,86.210000) (39.602941,86.210000) (41.441176,86.270000) (43.279412,86.330000) (45.117647,86.410000) (46.955882,86.410000) (48.794118,86.410000) (50.632353,86.540000) (52.470588,86.540000) (54.308824,86.540000) (56.147059,86.540000) (57.985294,86.540000) (59.823529,86.540000) (61.661765,86.540000) (63.500000,86.540000) (65.338235,86.540000) (67.176471,86.540000) (69.014706,86.540000) (70.852941,86.640000) (72.691176,86.640000) (74.529412,86.640000) (76.367647,86.640000) (78.205882,86.640000) (80.044118,86.640000)};
    \addplot coordinates {(2.838235,72.350000) (4.676471,77.660000) (6.514706,80.520000) (8.352941,81.720000) (10.191176,82.340000) (12.029412,83.310000) (13.867647,83.580000) (15.705882,84.340000) (17.544118,85.030000) (19.382353,85.030000) (21.220588,85.170000) (23.058824,85.470000) (24.897059,85.500000) (26.735294,86.010000) (28.573529,86.010000) (30.411765,86.100000) (32.250000,86.310000) (34.088235,86.480000) (35.926471,86.480000) (37.764706,86.480000) (39.602941,86.480000) (41.441176,86.480000) (43.279412,86.540000) (45.117647,86.540000) (46.955882,86.540000) (48.794118,86.540000) (50.632353,86.540000) (52.470588,86.540000) (54.308824,86.540000) (56.147059,86.540000) (57.985294,86.640000) (59.823529,86.640000) (61.661765,86.730000) (63.500000,86.730000) (65.338235,86.830000) (67.176471,86.830000) (69.014706,86.830000) (70.852941,86.830000) (72.691176,86.840000) (74.529412,86.840000) (76.367647,86.840000) (78.205882,86.840000) (80.044118,86.840000) (81.882353,86.840000)};
\addplot coordinates {(2.838235,75.140000) (4.676471,78.630000) (6.514706,80.560000) (8.352941,82.390000) (10.191176,83.340000) (12.029412,84.070000) (13.867647,84.530000) (15.705882,84.550000) (17.544118,84.950000) (19.382353,85.120000) (21.220588,85.120000) (23.058824,85.370000) (24.897059,85.620000) (26.735294,85.620000) (28.573529,85.740000) (30.411765,85.980000) (32.250000,85.980000) (34.088235,85.980000) (35.926471,86.400000) (37.764706,86.410000) (39.602941,86.410000) (41.441176,86.410000) (43.279412,86.410000) (45.117647,86.610000) (46.955882,86.610000) (48.794118,86.610000) (50.632353,86.610000) (52.470588,86.680000) (54.308824,86.680000) (56.147059,86.680000) (57.985294,86.760000) (59.823529,86.760000) (61.661765,86.760000) (63.500000,86.760000) (65.338235,86.920000) (67.176471,86.920000) (69.014706,86.920000) (70.852941,86.920000) (72.691176,86.920000) (74.529412,86.920000) (76.367647,86.920000)};
\addplot coordinates {(2.838235,69.730000) (4.676471,74.070000) (6.514706,76.300000) (8.352941,78.160000) (10.191176,78.850000) (12.029412,79.710000) (13.867647,80.690000) (15.705882,81.110000) (17.544118,81.410000) (19.382353,81.990000) (21.220588,82.260000) (23.058824,82.450000) (24.897059,82.450000) (26.735294,82.730000) (28.573529,83.320000) (30.411765,83.320000) (32.250000,83.320000) (34.088235,83.550000) (35.926471,83.550000) (37.764706,83.970000) (39.602941,84.260000) (41.441176,84.360000) (43.279412,84.360000) (45.117647,84.480000) (46.955882,84.710000) (48.794118,85.010000) (50.632353,85.190000) (52.470588,85.190000) (54.308824,85.190000) (56.147059,85.190000) (57.985294,85.430000) (59.823529,85.570000) (61.661765,85.570000) (63.500000,85.570000) (65.338235,85.570000) (67.176471,85.570000) (69.014706,85.570000) (72.691176,85.680000) (74.529412,85.680000) (76.367647,85.690000) (78.205882,85.960000) (80.044118,86.180000) (81.882353,86.180000)};
    \addplot[mark=none, dashed, samples=2, domain=-100:200] {86.86};
    \addplot[mark=none, loosely dashed, samples=2, domain=-100:200] {84};
	\legend{MNLP, LC, BALD, RAND, Best Deep Model, Best Shallow Model}
	\end{axis}
\end{tikzpicture}}
     \caption{OntoNotes-5.0 English}
     \label{fig:test-english}
   \end{subfigure}
   \hspace{1cm}
   \begin{subfigure}[t]{0.4\textwidth}
     \centering
%      \includegraphics[width=\linewidth]{active-zh-v2.pdf}
{\small \begin{tikzpicture}[scale=1]
	\begin{axis}[mark repeat=4, 
    legend pos=south east,
    legend style={nodes={scale=0.5, transform shape}},
        width=1.2\textwidth,
        height=0.9\textwidth,
		xlabel={Percent of words annotated},
		ylabel={Test F1 score}, xmin=-5, xmax=110]
\addplot coordinates {(3.645503,65.980000) (6.291005,69.640000) (8.936508,71.390000) (11.582011,72.710000) (14.227513,73.150000) (16.873016,74.070000) (19.518519,74.640000) (22.164021,74.640000) (24.809524,74.640000) (27.455026,74.640000) (30.100529,75.020000) (32.746032,75.020000) (35.391534,75.200000) (38.037037,75.760000) (40.682540,75.760000) (43.328042,75.760000) (45.973545,75.760000) (48.619048,75.760000) (51.264550,75.760000) (53.910053,75.760000) (56.555556,75.760000) (59.201058,75.760000) (61.846561,75.760000) (64.492063,75.760000) (67.137566,75.860000) (69.783069,75.860000) (72.428571,75.860000) (77.719577,75.860000) (80.365079,75.860000) (83.010582,75.860000) (85.656085,75.930000) (88.301587,75.930000) (90.947090,75.930000) (93.592593,75.970000) (96.238095,75.970000) (98.883598,75.970000) (101.529101,76.000000) (104.174603,76.000000)};
\addplot coordinates {(3.645503,64.950000) (6.291005,69.230000) (8.936508,70.310000) (11.582011,71.830000) (14.227513,72.020000) (16.873016,73.090000) (19.518519,73.250000) (22.164021,74.260000) (24.809524,74.480000) (27.455026,74.520000) (30.100529,75.240000) (32.746032,75.240000) (35.391534,75.350000) (38.037037,75.530000) (40.682540,75.530000) (43.328042,75.760000) (45.973545,75.760000) (48.619048,75.780000) (51.264550,75.780000) (53.910053,75.830000) (56.555556,76.020000) (59.201058,76.020000) (61.846561,76.020000) (64.492063,76.040000) (69.783069,76.190000) (72.428571,76.190000) (75.074074,76.190000) (77.719577,76.190000) (80.365079,76.190000) (83.010582,76.190000) (88.301587,76.190000) (90.947090,76.190000) (93.592593,76.190000) (96.238095,76.190000) (98.883598,76.190000) (101.529101,76.190000) (104.174603,76.190000) (106.820106,76.190000)};
\addplot coordinates {(3.645503,66.180000) (6.291005,69.760000) (8.936508,70.540000) (11.582011,71.900000) (14.227513,72.870000) (16.873016,73.530000) (19.518519,73.530000) (22.164021,73.730000) (24.809524,73.830000) (27.455026,74.510000) (30.100529,74.800000) (32.746032,75.110000) (35.391534,75.410000) (38.037037,75.610000) (40.682540,75.610000) (43.328042,75.610000) (45.973545,75.720000) (48.619048,75.720000) (51.264550,75.720000) (53.910053,75.720000) (56.555556,75.720000) (59.201058,75.720000) (61.846561,75.720000) (64.492063,75.850000) (67.137566,75.890000) (69.783069,75.890000) (72.428571,75.910000) (75.074074,75.910000) (77.719577,75.910000) (80.365079,75.910000) (83.010582,75.910000) (85.656085,75.910000) (88.301587,75.910000) (90.947090,75.910000) (93.592593,75.990000) (96.238095,75.990000) (98.883598,75.990000) (101.529101,75.990000)};
\addplot coordinates {(3.645503,63.390000) (6.291005,67.180000) (8.936508,68.710000) (11.582011,69.760000) (14.227513,70.720000) (16.873016,70.860000) (19.518519,71.260000) (22.164021,71.800000) (24.809524,72.150000) (27.455026,72.440000) (30.100529,72.760000) (32.746032,72.900000) (35.391534,72.900000) (38.037037,73.120000) (40.682540,73.340000) (43.328042,73.340000) (45.973545,73.890000) (48.619048,74.040000) (51.264550,74.040000) (53.910053,74.100000) (56.555556,74.100000) (59.201058,74.390000) (61.846561,74.640000) (64.492063,74.720000) (67.137566,74.740000) (69.783069,75.160000) (72.428571,75.160000) (75.074074,75.160000) (77.719577,75.160000) (80.365079,75.160000) (83.010582,75.280000) (85.656085,75.330000) (88.301587,75.520000) (90.947090,75.520000) (93.592593,75.520000) (96.238095,75.520000) (98.883598,75.520000)};
    \addplot[mark=none, dashed, samples=2, domain=-100:200] {75.63};
    \addplot[mark=none, loosely dashed, samples=2, domain=-100:200] {74};
	\legend{MNLP, LC, BALD, RAND, Best Deep Model, Best Shallow Model}
	\end{axis}
\end{tikzpicture}}
  \caption{OntoNotes-5.0 Chinese}
  \label{fig:test-chinese}
   \end{subfigure}
   \caption{F1 score on the test dataset, in terms of the number of words labeled.}
   \label{fig:active}
\end{figure*}

==> sections/0-definitions.tex <==
\RequirePackage{latexsym}
\RequirePackage{amsmath}
\let\proof\relax
\let\endproof\relax
\RequirePackage{amsthm}
\RequirePackage{amssymb}
\RequirePackage{bm}

%%%%%%%% Stock standard definitions %%%%%%%%%%%%%%%

\newcommand{\ab}{\mathbf{a}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\cbb}{\mathbf{c}}
\newcommand{\db}{\mathbf{d}}
\newcommand{\eb}{\mathbf{e}}
\newcommand{\fb}{\mathbf{f}}
\newcommand{\gb}{\mathbf{g}}
\newcommand{\hb}{\mathbf{h}}
\newcommand{\ib}{\mathbf{i}}
\newcommand{\jb}{\mathbf{j}}
\newcommand{\kb}{\mathbf{k}}
\newcommand{\lb}{\mathbf{l}}
\newcommand{\mb}{\mathbf{m}}
\newcommand{\nbb}{\mathbf{n}}
\newcommand{\ob}{\mathbf{o}}
\newcommand{\pb}{\mathbf{p}}
\newcommand{\qb}{\mathbf{q}}
\newcommand{\rb}{\mathbf{r}}
\newcommand{\sbb}{\mathbf{s}}
\newcommand{\tb}{\mathbf{t}}
\newcommand{\ub}{\mathbf{u}}
\newcommand{\vb}{\mathbf{v}}
\newcommand{\wb}{\mathbf{w}}
\newcommand{\xb}{\mathbf{x}}
\newcommand{\yb}{\mathbf{y}}
\newcommand{\zb}{\mathbf{z}}

\newcommand{\abtil}{\tilde{\ab}}
\newcommand{\bbtil}{\tilde{\bb}}
\newcommand{\cbtil}{\tilde{\cbb}}
\newcommand{\dbtil}{\tilde{\db}}
\newcommand{\ebtil}{\tilde{\eb}}
\newcommand{\fbtil}{\tilde{\fb}}
\newcommand{\gbtil}{\tilde{\gb}}
\newcommand{\hbtil}{\tilde{\hb}}
\newcommand{\ibtil}{\tilde{\ib}}
\newcommand{\jbtil}{\tilde{\jb}}
\newcommand{\kbtil}{\tilde{\kb}}
\newcommand{\lbtil}{\tilde{\lb}}
\newcommand{\mbtil}{\tilde{\mb}}
\newcommand{\nbtil}{\tilde{\nbb}}
\newcommand{\obtil}{\tilde{\ob}}
\newcommand{\pbtil}{\tilde{\pb}}
\newcommand{\qbtil}{\tilde{\qb}}
\newcommand{\rbtil}{\tilde{\rb}}
\newcommand{\sbtil}{\tilde{\sbb}}
\newcommand{\tbtil}{\tilde{\tb}}
\newcommand{\ubtil}{\tilde{\ub}}
\newcommand{\vbtil}{\tilde{\vb}}
\newcommand{\wbtil}{\tilde{\wb}}
\newcommand{\xbtil}{\tilde{\xb}}
\newcommand{\ybtil}{\tilde{\yb}}
\newcommand{\zbtil}{\tilde{\zb}}

\newcommand{\atil}{\tilde{a}}
\newcommand{\btil}{\tilde{b}}
\newcommand{\ctil}{\tilde{c}}
\newcommand{\dtil}{\tilde{d}}
\newcommand{\etil}{\tilde{e}}
\newcommand{\ftil}{\tilde{f}}
\newcommand{\gtil}{\tilde{g}}
\newcommand{\htil}{\tilde{h}}
\newcommand{\itil}{\tilde{i}}
\newcommand{\jtil}{\tilde{j}}
\newcommand{\ktil}{\tilde{k}}
\newcommand{\ltil}{\tilde{l}}
\newcommand{\mtil}{\tilde{m}}
\newcommand{\ntil}{\tilde{n}}
\newcommand{\otil}{\tilde{o}}
\newcommand{\ptil}{\tilde{p}}
\newcommand{\qtil}{\tilde{q}}
\newcommand{\rtil}{\tilde{r}}
\newcommand{\stil}{\tilde{s}}
\newcommand{\ttil}{\tilde{t}}
\newcommand{\util}{\tilde{u}}
\newcommand{\vtil}{\tilde{v}}
\newcommand{\wtil}{\tilde{w}}
\newcommand{\xtil}{\tilde{x}}
\newcommand{\ytil}{\tilde{y}}
\newcommand{\ztil}{\tilde{z}}

\newcommand{\ahat}{\hat{a}}
\newcommand{\bhat}{\hat{b}}
\newcommand{\chat}{\hat{c}}
\newcommand{\dhat}{\hat{d}}
\newcommand{\ehat}{\hat{e}}
\newcommand{\fhat}{\hat{f}}
\newcommand{\ghat}{\hat{g}}
\newcommand{\hhat}{\hat{h}}
\newcommand{\ihat}{\hat{i}}
\newcommand{\jhat}{\hat{j}}
\newcommand{\khat}{\hat{k}}
\newcommand{\lhat}{\hat{l}}
\newcommand{\mhat}{\hat{m}}
\newcommand{\nhat}{\hat{n}}
\newcommand{\ohat}{\hat{o}}
\newcommand{\phat}{\hat{p}}
\newcommand{\qhat}{\hat{q}}
\newcommand{\rhat}{\hat{r}}
\newcommand{\shat}{\hat{s}}
\newcommand{\that}{\hat{t}}
\newcommand{\uhat}{\hat{u}}
\newcommand{\vhat}{\hat{v}}
\newcommand{\what}{\hat{w}}
\newcommand{\xhat}{\hat{x}}
\newcommand{\yhat}{\hat{y}}
\newcommand{\zhat}{\hat{z}}

\newcommand{\abhat}{\hat{\ab}}
\newcommand{\bbhat}{\hat{\bb}}
\newcommand{\cbhat}{\hat{\cb}}
\newcommand{\dbhat}{\hat{\db}}
\newcommand{\ebhat}{\hat{\eb}}
\newcommand{\fbhat}{\hat{\fb}}
\newcommand{\gbhat}{\hat{\gb}}
\newcommand{\hbhat}{\hat{\hb}}
\newcommand{\ibhat}{\hat{\ib}}
\newcommand{\jbhat}{\hat{\jb}}
\newcommand{\kbhat}{\hat{\kb}}
\newcommand{\lbhat}{\hat{\lb}}
\newcommand{\mbhat}{\hat{\mb}}
\newcommand{\nbhat}{\hat{\nb}}
\newcommand{\obhat}{\hat{\ob}}
\newcommand{\pbhat}{\hat{\pb}}
\newcommand{\qbhat}{\hat{\qb}}
\newcommand{\rbhat}{\hat{\rb}}
\newcommand{\sbhat}{\hat{\sb}}
\newcommand{\tbhat}{\hat{\tb}}
\newcommand{\ubhat}{\hat{\ub}}
\newcommand{\vbhat}{\hat{\vb}}
\newcommand{\wbhat}{\hat{\wb}}
\newcommand{\xbhat}{\hat{\xb}}
\newcommand{\ybhat}{\hat{\yb}}
\newcommand{\zbhat}{\hat{\zb}}

\newcommand{\Atil}{\tilde{A}}
\newcommand{\Btil}{\tilde{B}}
\newcommand{\Ctil}{\tilde{C}}
\newcommand{\Dtil}{\tilde{D}}
\newcommand{\Etil}{\tilde{E}}
\newcommand{\Ftil}{\tilde{F}}
\newcommand{\Gtil}{\tilde{G}}
\newcommand{\Htil}{\tilde{H}}
\newcommand{\Itil}{\tilde{I}}
\newcommand{\Jtil}{\tilde{J}}
\newcommand{\Ktil}{\tilde{K}}
\newcommand{\Ltil}{\tilde{L}}
\newcommand{\Mtil}{\tilde{M}}
\newcommand{\Ntil}{\tilde{N}}
\newcommand{\Otil}{\tilde{O}}
\newcommand{\Ptil}{\tilde{P}}
\newcommand{\Qtil}{\tilde{Q}}
\newcommand{\Rtil}{\tilde{R}}
\newcommand{\Stil}{\tilde{S}}
\newcommand{\Ttil}{\tilde{T}}
\newcommand{\Util}{\tilde{U}}
\newcommand{\Vtil}{\tilde{V}}
\newcommand{\Wtil}{\tilde{W}}
\newcommand{\Xtil}{\tilde{X}}
\newcommand{\Ytil}{\tilde{Y}}
\newcommand{\Ztil}{\tilde{Z}}

\newcommand{\abar}{\bar{a}}
\newcommand{\bbar}{\bar{b}}
\newcommand{\cbar}{\bar{c}}
\newcommand{\dbar}{\bar{d}}
\newcommand{\ebar}{\bar{e}}
\newcommand{\fbar}{\bar{f}}
\newcommand{\gbar}{\bar{g}}
\newcommand{\hbr}{\bar{h}}
\newcommand{\ibar}{\bar{i}}
\newcommand{\jbar}{\bar{j}}
\newcommand{\kbar}{\bar{k}}
\newcommand{\lbar}{\bar{l}}
\newcommand{\mbar}{\bar{m}}
\newcommand{\nbar}{\bar{n}}
\newcommand{\obar}{\bar{o}}
\newcommand{\pbar}{\bar{p}}
\newcommand{\qbar}{\bar{q}}
\newcommand{\rbar}{\bar{r}}
\newcommand{\sbar}{\bar{s}}
\newcommand{\tbar}{\bar{t}}
\newcommand{\ubar}{\bar{u}}
\newcommand{\vbar}{\bar{v}}
\newcommand{\wbar}{\bar{w}}
\newcommand{\xbar}{\bar{x}}
\newcommand{\ybar}{\bar{y}}
\newcommand{\zbar}{\bar{z}}

\newcommand{\abbar}{\bar{\ab}}
\newcommand{\bbbar}{\bar{\bb}}
\newcommand{\cbbar}{\bar{\cb}}
\newcommand{\dbbar}{\bar{\db}}
\newcommand{\ebbar}{\bar{\eb}}
\newcommand{\fbbar}{\bar{\fb}}
\newcommand{\gbbar}{\bar{\gb}}
\newcommand{\hbbar}{\bar{\hb}}
\newcommand{\ibbar}{\bar{\ib}}
\newcommand{\jbbar}{\bar{\jb}}
\newcommand{\kbbar}{\bar{\kb}}
\newcommand{\lbbar}{\bar{\lb}}
\newcommand{\mbbar}{\bar{\mb}}
\newcommand{\nbbar}{\bar{\nbb}}
\newcommand{\obbar}{\bar{\ob}}
\newcommand{\pbbar}{\bar{\pb}}
\newcommand{\qbbar}{\bar{\qb}}
\newcommand{\rbbar}{\bar{\rb}}
\newcommand{\sbbar}{\bar{\sbb}}
\newcommand{\tbbar}{\bar{\tb}}
\newcommand{\ubbar}{\bar{\ub}}
\newcommand{\vbbar}{\bar{\vb}}
\newcommand{\wbbar}{\bar{\wb}}
\newcommand{\xbbar}{\bar{\xb}}
\newcommand{\ybbar}{\bar{\yb}}
\newcommand{\zbbar}{\bar{\zb}}

\newcommand{\Ab}{\mathbf{A}}
\newcommand{\Bb}{\mathbf{B}}
\newcommand{\Cb}{\mathbf{C}}
\newcommand{\Db}{\mathbf{D}}
\newcommand{\Eb}{\mathbf{E}}
\newcommand{\Fb}{\mathbf{F}}
\newcommand{\Gb}{\mathbf{G}}
\newcommand{\Hb}{\mathbf{H}}
\newcommand{\Ib}{\mathbf{I}}
\newcommand{\Jb}{\mathbf{J}}
\newcommand{\Kb}{\mathbf{K}}
\newcommand{\Lb}{\mathbf{L}}
\newcommand{\Mb}{\mathbf{M}}
\newcommand{\Nb}{\mathbf{N}}
\newcommand{\Ob}{\mathbf{O}}
\newcommand{\Pb}{\mathbf{P}}
\newcommand{\Qb}{\mathbf{Q}}
\newcommand{\Rb}{\mathbf{R}}
\newcommand{\Sbb}{\mathbf{S}}
\newcommand{\Tb}{\mathbf{T}}
\newcommand{\Ub}{\mathbf{U}}
\newcommand{\Vb}{\mathbf{V}}
\newcommand{\Wb}{\mathbf{W}}
\newcommand{\Xb}{\mathbf{X}}
\newcommand{\Yb}{\mathbf{Y}}
\newcommand{\Zb}{\mathbf{Z}}

\newcommand{\Abtil}{\tilde{\Ab}}
\newcommand{\Bbtil}{\tilde{\Bb}}
\newcommand{\Cbtil}{\tilde{\Cb}}
\newcommand{\Dbtil}{\tilde{\Db}}
\newcommand{\Ebtil}{\tilde{\Eb}}
\newcommand{\Fbtil}{\tilde{\Fb}}
\newcommand{\Gbtil}{\tilde{\Gb}}
\newcommand{\Hbtil}{\tilde{\Hb}}
\newcommand{\Ibtil}{\tilde{\Ib}}
\newcommand{\Jbtil}{\tilde{\Jb}}
\newcommand{\Kbtil}{\tilde{\Kb}}
\newcommand{\Lbtil}{\tilde{\Lb}}
\newcommand{\Mbtil}{\tilde{\Mb}}
\newcommand{\Nbtil}{\tilde{\Nb}}
\newcommand{\Obtil}{\tilde{\Ob}}
\newcommand{\Pbtil}{\tilde{\Pb}}
\newcommand{\Qbtil}{\tilde{\Qb}}
\newcommand{\Rbtil}{\tilde{\Rb}}
\newcommand{\Sbtil}{\tilde{\Sbb}}
\newcommand{\Tbtil}{\tilde{\Tb}}
\newcommand{\Ubtil}{\tilde{\Ub}}
\newcommand{\Vbtil}{\tilde{\Vb}}
\newcommand{\Wbtil}{\tilde{\Wb}}
\newcommand{\Xbtil}{\tilde{\Xb}}
\newcommand{\Ybtil}{\tilde{\Yb}}
\newcommand{\Zbtil}{\tilde{\Zb}}

\newcommand{\Abar}{\bar{A}}
\newcommand{\Bbar}{\bar{B}}
\newcommand{\Cbar}{\bar{C}}
\newcommand{\Dbar}{\bar{D}}
\newcommand{\Ebar}{\bar{E}}
\newcommand{\Fbar}{\bar{F}}
\newcommand{\Gbar}{\bar{G}}
\newcommand{\Hbar}{\bar{H}}
\newcommand{\Ibar}{\bar{I}}
\newcommand{\Jbar}{\bar{J}}
\newcommand{\Kbar}{\bar{K}}
\newcommand{\Lbar}{\bar{L}}
\newcommand{\Mbar}{\bar{M}}
\newcommand{\Nbar}{\bar{N}}
\newcommand{\Obar}{\bar{O}}
\newcommand{\Pbar}{\bar{P}}
\newcommand{\Qbar}{\bar{Q}}
\newcommand{\Rbar}{\bar{R}}
\newcommand{\Sbar}{\bar{S}}
\newcommand{\Tbar}{\bar{T}}
\newcommand{\Ubar}{\bar{U}}
\newcommand{\Vbar}{\bar{V}}
\newcommand{\Wbar}{\bar{W}}
\newcommand{\Xbar}{\bar{X}}
\newcommand{\Ybar}{\bar{Y}}
\newcommand{\Zbar}{\bar{Z}}

\newcommand{\Abbar}{\bar{\Ab}}
\newcommand{\Bbbar}{\bar{\Bb}}
\newcommand{\Cbbar}{\bar{\Cb}}
\newcommand{\Dbbar}{\bar{\Db}}
\newcommand{\Ebbar}{\bar{\Eb}}
\newcommand{\Fbbar}{\bar{\Fb}}
\newcommand{\Gbbar}{\bar{\Gb}}
\newcommand{\Hbbar}{\bar{\Hb}}
\newcommand{\Ibbar}{\bar{\Ib}}
\newcommand{\Jbbar}{\bar{\Jb}}
\newcommand{\Kbbar}{\bar{\Kb}}
\newcommand{\Lbbar}{\bar{\Lb}}
\newcommand{\Mbbar}{\bar{\Mb}}
\newcommand{\Nbbar}{\bar{\Nb}}
\newcommand{\Obbar}{\bar{\Ob}}
\newcommand{\Pbbar}{\bar{\Pb}}
\newcommand{\Qbbar}{\bar{\Qb}}
\newcommand{\Rbbar}{\bar{\Rb}}
\newcommand{\Sbbar}{\bar{\Sb}}
\newcommand{\Tbbar}{\bar{\Tb}}
\newcommand{\Ubbar}{\bar{\Ub}}
\newcommand{\Vbbar}{\bar{\Vb}}
\newcommand{\Wbbar}{\bar{\Wb}}
\newcommand{\Xbbar}{\bar{\Xb}}
\newcommand{\Ybbar}{\bar{\Yb}}
\newcommand{\Zbbar}{\bar{\Zb}}

\newcommand{\Ahat}{\hat{A}}
\newcommand{\Bhat}{\hat{B}}
\newcommand{\Chat}{\hat{C}}
\newcommand{\Dhat}{\hat{D}}
\newcommand{\Ehat}{\hat{E}}
\newcommand{\Fhat}{\hat{F}}
\newcommand{\Ghat}{\hat{G}}
\newcommand{\Hhat}{\hat{H}}
\newcommand{\Ihat}{\hat{I}}
\newcommand{\Jhat}{\hat{J}}
\newcommand{\Khat}{\hat{K}}
\newcommand{\Lhat}{\hat{L}}
\newcommand{\Mhat}{\hat{M}}
\newcommand{\Nhat}{\hat{N}}
\newcommand{\Ohat}{\hat{O}}
\newcommand{\Phat}{\hat{P}}
\newcommand{\Qhat}{\hat{Q}}
\newcommand{\Rhat}{\hat{R}}
\newcommand{\Shat}{\hat{S}}
\newcommand{\That}{\hat{T}}
\newcommand{\Uhat}{\hat{U}}
\newcommand{\Vhat}{\hat{V}}
\newcommand{\What}{\hat{W}}
\newcommand{\Xhat}{\hat{X}}
\newcommand{\Yhat}{\hat{Y}}
\newcommand{\Zhat}{\hat{Z}}

\newcommand{\Abhat}{\hat{\Ab}}
\newcommand{\Bbhat}{\hat{\Bb}}
\newcommand{\Cbhat}{\hat{\Cb}}
\newcommand{\Dbhat}{\hat{\Db}}
\newcommand{\Ebhat}{\hat{\Eb}}
\newcommand{\Fbhat}{\hat{\Fb}}
\newcommand{\Gbhat}{\hat{\Gb}}
\newcommand{\Hbhat}{\hat{\Hb}}
\newcommand{\Ibhat}{\hat{\Ib}}
\newcommand{\Jbhat}{\hat{\Jb}}
\newcommand{\Kbhat}{\hat{\Kb}}
\newcommand{\Lbhat}{\hat{\Lb}}
\newcommand{\Mbhat}{\hat{\Mb}}
\newcommand{\Nbhat}{\hat{\Nb}}
\newcommand{\Obhat}{\hat{\Ob}}
\newcommand{\Pbhat}{\hat{\Pb}}
\newcommand{\Qbhat}{\hat{\Qb}}
\newcommand{\Rbhat}{\hat{\Rb}}
\newcommand{\Sbhat}{\hat{\Sb}}
\newcommand{\Tbhat}{\hat{\Tb}}
\newcommand{\Ubhat}{\hat{\Ub}}
\newcommand{\Vbhat}{\hat{\Vb}}
\newcommand{\Wbhat}{\hat{\Wb}}
\newcommand{\Xbhat}{\hat{\Xb}}
\newcommand{\Ybhat}{\hat{\Yb}}
\newcommand{\Zbhat}{\hat{\Zb}}

\newcommand{\Acal}{\mathcal{A}}
\newcommand{\Bcal}{\mathcal{B}}
\newcommand{\Ccal}{\mathcal{C}}
\newcommand{\Dcal}{\mathcal{D}}
\newcommand{\Ecal}{\mathcal{E}}
\newcommand{\Fcal}{\mathcal{F}}
\newcommand{\Gcal}{\mathcal{G}}
\newcommand{\Hcal}{\mathcal{H}}
\newcommand{\Ical}{\mathcal{I}}
\newcommand{\Jcal}{\mathcal{J}}
\newcommand{\Kcal}{\mathcal{K}}
\newcommand{\Lcal}{\mathcal{L}}
\newcommand{\Mcal}{\mathcal{M}}
\newcommand{\Ncal}{\mathcal{N}}
\newcommand{\Ocal}{\mathcal{O}}
\newcommand{\Pcal}{\mathcal{P}}
\newcommand{\Qcal}{\mathcal{Q}}
\newcommand{\Rcal}{\mathcal{R}}
\newcommand{\Scal}{{\mathcal{S}}}
\newcommand{\Tcal}{{\mathcal{T}}}
\newcommand{\Ucal}{\mathcal{U}}
\newcommand{\Vcal}{\mathcal{V}}
\newcommand{\Wcal}{\mathcal{W}}
\newcommand{\Xcal}{\mathcal{X}}
\newcommand{\Ycal}{\mathcal{Y}}
\newcommand{\Zcal}{\mathcal{Z}}

\newcommand{\Atilde}{\widetilde{A}}
\newcommand{\Btilde}{\widetilde{B}}
\newcommand{\Ctilde}{\widetilde{C}}
\newcommand{\Dtilde}{\widetilde{D}}
\newcommand{\Etilde}{\widetilde{E}}
\newcommand{\Ftilde}{\widetilde{F}}
\newcommand{\Gtilde}{\widetilde{G}}
\newcommand{\Htilde}{\widetilde{H}}
\newcommand{\Itilde}{\widetilde{I}}
\newcommand{\Jtilde}{\widetilde{J}}
\newcommand{\Ktilde}{\widetilde{K}}
\newcommand{\Ltilde}{\widetilde{L}}
\newcommand{\Mtilde}{\widetilde{M}}
\newcommand{\Ntilde}{\widetilde{N}}
\newcommand{\Otilde}{\widetilde{O}}
\newcommand{\Ptilde}{\widetilde{P}}
\newcommand{\Qtilde}{\widetilde{Q}}
\newcommand{\Rtilde}{\widetilde{R}}
\newcommand{\Stilde}{\widetilde{S}}
\newcommand{\Ttilde}{\widetilde{T}}
\newcommand{\Utilde}{\widetilde{U}}
\newcommand{\Vtilde}{\widetilde{V}}
\newcommand{\Wtilde}{\widetilde{W}}
\newcommand{\Xtilde}{\widetilde{X}}
\newcommand{\Ytilde}{\widetilde{Y}}
\newcommand{\Ztilde}{\widetilde{Z}}

\renewcommand{\vec}[1]{\mathbf{\boldsymbol{#1}}}

\newcommand{\avec}{\vec{a}}
\newcommand{\bvec}{\vec{b}}
\newcommand{\cvec}{\vec{c}}
\newcommand{\dvec}{\vec{d}}
\newcommand{\evec}{\vec{e}}
\newcommand{\fvec}{\vec{f}}
\newcommand{\gvec}{\vec{g}}
\newcommand{\hvec}{\vec{h}}
\newcommand{\ivec}{\vec{i}}
\newcommand{\jvec}{\vec{j}}
\newcommand{\kvec}{\vec{k}}
\newcommand{\lvec}{\vec{l}}
\newcommand{\mvec}{\vec{m}}
\newcommand{\nvec}{\vec{n}}
\newcommand{\ovec}{\vec{o}}
\newcommand{\pvec}{\vec{p}}
\newcommand{\qvec}{\vec{q}}
\newcommand{\rvec}{\vec{r}}
\newcommand{\svec}{\vec{s}}
\newcommand{\tvec}{\vec{t}}
\newcommand{\uvec}{\vec{u}}
\newcommand{\vvec}{\vec{v}}
\newcommand{\wvec}{\vec{w}}
\newcommand{\xvec}{\vec{x}}
\newcommand{\yvec}{\vec{y}}
\newcommand{\zvec}{\vec{z}}

\newcommand{\va}{\vec{a}}
\newcommand{\vecb}{\vec{b}}
\newcommand{\vc}{\vec{c}}
\newcommand{\vd}{\vec{d}}
\newcommand{\veee}{\vec{e}}
\newcommand{\vf}{\vec{f}}
\newcommand{\vg}{\vec{g}}
\newcommand{\vh}{\vec{h}}
\newcommand{\vi}{\vec{i}}
\newcommand{\vo}{\vec{o}}
\newcommand{\vp}{\vec{p}}
\newcommand{\vq}{\vec{q}}
\newcommand{\vr}{\vec{r}}
\newcommand{\vs}{\vec{s}}
\newcommand{\vt}{\vec{t}}
\newcommand{\vu}{\vec{u}}
\newcommand{\vv}{\vec{v}}
\newcommand{\vx}{\vec{x}}
\newcommand{\vw}{\vec{w}}
\newcommand{\vy}{\vec{y}}
\newcommand{\vz}{\vec{z}}

\newcommand{\Avec}{\vec{A}}
\newcommand{\Bvec}{\vec{B}}
\newcommand{\Cvec}{\vec{C}}
\newcommand{\Dvec}{\vec{D}}
\newcommand{\Evec}{\vec{E}}
\newcommand{\Fvec}{\vec{F}}
\newcommand{\Gvec}{\vec{G}}
\newcommand{\Hvec}{\vec{H}}
\newcommand{\Ivec}{\vec{I}}
\newcommand{\Jvec}{\vec{J}}
\newcommand{\Kvec}{\vec{K}}
\newcommand{\Lvec}{\vec{L}}
\newcommand{\Mvec}{\vec{M}}
\newcommand{\Nvec}{\vec{N}}
\newcommand{\Ovec}{\vec{O}}
\newcommand{\Pvec}{\vec{P}}
\newcommand{\Qvec}{\vec{Q}}
\newcommand{\Rvec}{\vec{R}}
\newcommand{\Svec}{\vec{S}}
\newcommand{\Tvec}{\vec{T}}
\newcommand{\Uvec}{\vec{U}}
\newcommand{\Vvec}{\vec{V}}
\newcommand{\Wvec}{\vec{W}}
\newcommand{\Xvec}{\vec{X}}
\newcommand{\Yvec}{\vec{Y}}
\newcommand{\Zvec}{\vec{Z}}

\newcommand{\Amat}{\Ab}
\newcommand{\Bmat}{\Bb}
\newcommand{\Cmat}{\Cb}
\newcommand{\Dmat}{\Db}
\newcommand{\Emat}{\Eb}
\newcommand{\Fmat}{\Fb}
\newcommand{\Gmat}{\Gb}
\newcommand{\Hmat}{\Hb}
\newcommand{\Imat}{\Ib}

\newcommand{\Vmat}{\Vb}
\newcommand{\Wmat}{\Wb}
\newcommand{\Xmat}{\Xb}
\newcommand{\Ymat}{\Yb}
\newcommand{\Zmat}{\Zb}


\newcommand{\yvecbar}{\bar{\vec{y}}}
\newcommand{\wvecbar}{\bar{\vec{w}}}
\newcommand{\xvecbar}{\bar{\vec{x}}}
\newcommand{\yvectil}{\tilde{\vec{y}}}
\newcommand{\yvechat}{\hat{\vec{y}}}



% \renewcommand{\qedsymbol}{$\blacksquare$}


%%%%%%%% Widely accepted Sets and Symbols %%%%%%%%%%%%%%%

\newcommand{\CC}{\mathbb{C}} % Complex numbers
\newcommand{\EE}{\mathbb{E}} % Expectation
\newcommand{\FF}{\mathbb{F}} % Fexpectation
\newcommand{\HH}{\mathbb{H}} % Arbitrary field
\newcommand{\II}{\mathbb{I}} % Delta Indicator
\newcommand{\KK}{\mathbb{K}} % Arbitrary field
\newcommand{\MM}{\mathbb{M}} % Median
\newcommand{\NN}{\mathbb{N}} % Natural numbers
\newcommand{\PP}{\mathbb{P}} % Probability
\newcommand{\QQ}{\mathbb{Q}} % Rationals
\newcommand{\RR}{\mathbb{R}} % Real numbers
\newcommand{\RRbar}{\overline{\RR}} % Real numbers
\newcommand{\SSS}{\mathbb{S}}
\newcommand{\TT}{\mathbb{T}}
\newcommand{\VV}{\mathbb{V}} % Variance
\newcommand{\XX}{\mathbb{X}}
\newcommand{\YY}{\mathbb{Y}}
\newcommand{\ZZ}{\mathbb{Z}} % Integers

%%%%%%%% Mathematical Operations %%%%%%%%%%%%%%%

\newcommand*{\mini}{\mathop{\mathrm{minimize}}}
\newcommand*{\maxi}{\mathop{\mathrm{maximize}}}
\newcommand*{\argmin}{\mathop{\mathrm{argmin}}}
\newcommand*{\argmax}{\mathop{\mathrm{argmax}}}
\newcommand*{\arginf}{\mathop{\mathrm{arginf}}}
\newcommand*{\argsup}{\mathop{\mathrm{argsup}}}
\newcommand{\sgn}{\mathop{\mathrm{sign}}}
\newcommand{\tr}{\mathop{\mathrm{tr}}}
\newcommand{\diag}{\mathop{\mathrm{diag}}}
\newcommand{\rank}{\mathop{\mathrm{rank}}}
\newcommand{\vect}{\mathop{\mathrm{vec}}}
\newcommand{\traj}{\mathop{\mathrm{Traj}}}
\newcommand{\cov}{\mathrm{Cov}}
\newcommand{\conv}{\mathrm{conv}}
\newcommand{\const}{\mathrm{constant}}
\newcommand{\dom}{\mathop{\mathrm{dom}}}
\newcommand{\ri}{\mathop{\mathrm{ri}}}
\newcommand{\cl}{\mathop{\mathrm{cl}}}
\newcommand{\intr}{\mathop{\mathrm{int}}}
\newcommand{\bd}{\mathop{\mathrm{bd}}}
\newcommand{\emp}{\mathop{\mathrm{emp}}}
\newcommand{\core}{\mathop{\mathrm{core}}}
\newcommand{\co}{\mathop{\mathrm{co}}}
\newcommand{\nnz}{\mathop{\mathrm{nnz}}}
\newcommand{\eproof}{$\null\hfill\blacksquare$}

%%%%%%%% Utility functions %%%%%%%%%%%%%%%

\newcommand{\eq}[1]{(\ref{#1})}
\newcommand{\mymatrix}[2]{\left[\begin{array}{#1} #2 \end{array}\right]}
\newcommand{\mychoose}[2]{\left(\begin{array}{c} #1 \\ #2 \end{array}\right)}
\newcommand{\mydet}[1]{\det\left[ #1 \right]}
\newcommand{\myspan}[1]{\mathrm{span}\cbr{#1}}
\newcommand{\smallfrac}[2]{{\textstyle \frac{#1}{#2}}}
\newcommand{\pwrt}[1]{\frac{\partial}{\partial #1}}
\newcommand{\ppwrt}[1]{\frac{\partial^2}{(\partial #1)^2}}
\newcommand{\aleq}{\preccurlyeq}
\newcommand{\ageq}{\succcurlyeq}

%%%%%%%% Short Forms %%%%%%%%%%%%%%%

\newcommand{\ea}{\emph{et al.}}
\newcommand{\eg}{\emph{e.g.}}
\newcommand{\ie}{\emph{i.e.}}
\newcommand{\iid}{\emph{iid}}
\newcommand{\cf}{\emph{cf.}\ }
\newcommand{\wrt}{\emph{w.r.t.}\ }

%%%%%%%% Brackets %%%%%%%%%%%%%%%

\newcommand{\rbr}[1]{\left(#1\right)}
\newcommand{\sbr}[1]{\left[#1\right]}
\newcommand{\cbr}[1]{\left\{#1\right\}}
\newcommand{\nbr}[1]{\left\|#1\right\|}
\newcommand{\abr}[1]{\left|#1\right|}
\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}
\newcommand{\inner}[2]{\left\langle #1,#2 \right\rangle}
\newcommand{\norm}[1]{\|#1\|}
\newcommand{\ccc}[1]{|\!|\!|#1|\!|\!|}
\newcommand{\sembrack}[1]{[\![#1]\!]}

%%%%%%%%%%%%%%%  Mathematical Constants  %%%%%%%%%%%%%%%

\newcommand{\one}{\mathbf{1}}  % Identity
\newcommand{\zero}{\mathbf{0}} % Zero
\newcommand{\ind}{\boldsymbol{\mathsf{I}}}
\newcommand{\half}{\frac{1}{2}}
\newcommand{\sqrttwo}{\sqrt{2}}
\newcommand{\invsqrttwo}{\frac{1}{\sqrt{2}}}
\newcommand{\rmd}{\ensuremath{\mathrm{d}}}

%%%%%%%% Greek Symbols %%%%%%%%%%%%%%%

\newcommand{\sigmab}{\bm{\sigma}}
\newcommand{\Sigmab}{\mathbf{\Sigma}}

\newcommand{\val}{\vec{\alpha}}
\newcommand{\vbeta}{\vec{\beta}}
\newcommand{\vde}{\vec{\delta}}
\newcommand{\vga}{\vec{\gamma}}
\newcommand{\vsig}{\vec{\sigma}}
\newcommand{\vth}{\vec{\theta}}
\newcommand{\veta}{\vec{\eta}}
\newcommand{\vnu}{\vec{\nu}}
\newcommand{\vpsi}{\vec{\psi}}
\newcommand{\vpi}{\vec{\pi}}
\newcommand{\vphi}{\vec{\phi}}
\newcommand{\vxi}{\vec{\xi}}
\newcommand{\vze}{\vec{\zeta}}

\newcommand{\valbar}{\bar{\val}}
\newcommand{\valhat}{\hat{\val}}
\newcommand{\valtil}{\tilde{\val}}
\newcommand{\vthtil}{\tilde{\vth}}
\newcommand{\vthhat}{\hat{\vth}}
\newcommand{\vthbar}{\bar{\vth}}
\newcommand{\vbetatil}{\tilde{\vbeta}}
\newcommand{\vbetahat}{\hat{\vbeta}}

\newcommand{\alphavec}{\val}
\newcommand{\alphavecbar}{\bar{\val}}
\newcommand{\alphavechat}{\hat{\val}}
\newcommand{\alphavectil}{\tilde{\val}}
\newcommand{\betavec}{\vec{\beta}}
\newcommand{\gammavec}{\vec{\gamma}}
\newcommand{\deltavec}{\vec{\delta}}
\newcommand{\etavec}{\vec{\eta}}
\newcommand{\phivec}{\vec{\phi}}
\newcommand{\psivec}{\vec{\psi}}
\newcommand{\thetavec}{\vec{\theta}}
\newcommand{\muvec}{\vec{\mu}}
\newcommand{\xivec}{\vec{\xi}}
\newcommand{\chivec}{\vec{\chi}}
\newcommand{\lambdavec}{\vec{\lambda}}

\newcommand{\alphab}{\boldsymbol{\alpha}}
\newcommand{\betab}{\boldsymbol{\beta}}
\newcommand{\gammab}{\boldsymbol{\gamma}}
\newcommand{\thetab}{\boldsymbol{\theta}}
\newcommand{\mub}{\boldsymbol{\mu}}
\newcommand{\xib}{\boldsymbol{\xi}}
\newcommand{\Deltab}{\boldsymbol{\Delta}}
\newcommand{\Pib}{\boldsymbol{\Pi}}
\newcommand{\etab}{\boldsymbol{\eta}}
\newcommand{\taub}{\boldsymbol{\tau}}
\newcommand{\lambdab}{\boldsymbol{\lambda}}
\newcommand{\pitil}{\tilde{\pi}}
\newcommand{\elltil}{\tilde{\ell}}
\newcommand{\rhob}{\boldsymbol{\rho}}

\newcommand{\delhat}{\hat{\delta}}
\newcommand{\phihat}{\hat{\phi}}
\newcommand{\delbar}{\bar{\delta}}
\newcommand{\alphahat}{\hat{\alpha}}
\newcommand{\alphatil}{\tilde{\alpha}}
\newcommand{\mubar}{\bar{\mu}}
\newcommand{\thetahat}{\hat{\theta}}
\newcommand{\thetabar}{\bar{\theta}}
\newcommand{\betahat}{\hat{\beta}}

\newcommand{\xibar}{\bar{\xi}}
\newcommand{\lambdavectil}{\tilde{\vec{\lambda}}}
\newcommand{\thetatil}{\tilde{\theta}}
\newcommand{\betatil}{\tilde{\beta}}

\newcommand{\Omegabar}{\bar{\Omega}}

%%%% Symbols specific to this project %%%%%

\newcommand{\Poisson}{\mathrm{Poisson}}
\newcommand{\trank}{\text{rank}}
\newcommand{\otrank}{\overline{\text{rank}}}

